A Quantal Response Analysis of Defender-Attacker Sequential Security Games

We explore a scenario involving two sites and a sequential game between a defender and an attacker, where the defender is responsible for securing the sites while the attacker aims to attack them. Each site holds a loss value for the defender when compromised, along with a probability of successful attack. The defender can reduce these probabilities through security investments at each site. The attacker's objective is to target the site that maximizes the expected loss for the defender, taking into account the defender's security investments. While previous studies have examined security investments in such scenarios, our work investigates the impact of bounded rationality exhibited by the defender, as identified in behavioral economics. Specifically, we consider quantal behavioral bias, where humans make errors in selecting efficient (pure) strategies. We demonstrate the existence of a quantal response equilibrium in our sequential game and analyze how this bias affects the defender's choice of optimal security investments. Additionally, we quantify the inefficiency of equilibrium investments under quantal decision-making compared to an optimal solution devoid of behavioral biases. We provide numerical simulations to validate our main findings.

==> Bound_under_Behavioral_decisions.tex <==
\section{Bound on Behavioral Inefficiency}
In this section, we seek to define a measure to capture the inefficiency of the security investments due to the defender's behavioral decision-making. We thus define the Price of Behavioral Probability Weighting (PoBW) as the ratio of the {\it true} expected loss of the behavioral defender (under the behavioral investments) to the true expected loss of a non-behavioral defender. This notion is similar to the Price of Behavioral Anarchy (PoBA) metric introduced in \cite{abdallah2020behavioralnew}, which measured the inefficiency of game-theoretic equilibria with multiple behavioral defenders (similar to how the classical notion of Price of Anarchy measures the inefficiency of game-theoretic equilibria compared to a socially optimal solution~\cite{roughgarden2003price}).
% \footnote{SS: put citation to PoA here. Mus: done}
Here, PoBW measures only the inefficiency of the single defender due to her behavioral decision-making. Specifically, we define the Price of Behavioral Probability Weighting (PoBW) as
\begin{equation}\label{eq: Security Under Anarchy}
    PoBW = \frac{  L(\hat{r})}{L(r^*)},
\end{equation}
where $\hat{r} = \displaystyle \min_{r\in [0,R]} \max\{w(p_{1}(r)), A w\left(p_{2}(R - r)\right)\}$ and $r^* = \displaystyle \min_{r\in [0,R]} \max\{p_{1}(r), A p_{2}(R - r)\}$ denote the behavioral and non-behavioral defender's investments, respectively. We emphasize that the expected losses in both the numerator and the denominator are the \emph{true} (rather than perceived) expected losses (defined in \eqref{eq: Non_Behavioral_defender_expected_loss}) of the defender.

Now, we will establish the upper bound on the PoBW. We show that the PoBW is bounded if the total budget is bounded (regardless of the defender's behavioral level).

\begin{proposition}\label{prop:POBW_upper_bound}
Let the budget available to the defender be $R$, and let the probability of successful attack on sites $1$ and $2$ be given by $p_{1}(r)=e^{-r}$ and $p_{2}(r)=e^{-(R-r)}$, respectively. Then, for any $A$ and any behavioral level $\alpha \in (0,1]$,  $PoBW\leq \max\{A, \frac{1}{A}\} \exp(R)$. 
%\footnote{SS: don't understand what this $k$ means Mus: Replaced it as you suggested with $\max\{A, \frac{1}{A}\}$}. 
\end{proposition}
\begin{proof}
%First, consider the three corner cases: if $A = 0$,\footnote{SS: do you need to consider this?  You had defined $A > 0$ in the model.  Also, the bound becomes infinite in this case.  Just remove this case. Mus: Removed.} we then have $\hat{r} = r^* = R$. Thus, substituting in \eqref{eq: Security Under Anarchy} yields that we have $PoBW = 1$. 
%Similarly, if $A \to \infty$, we have $\hat{r} = r^* = 0$ and thus we have $PoBW = 1$. Moreover, if $A =  1$, we have $\hat{r} = r^*$ (from Theorem~\ref{thm: difference_equilibrium_behav_non_behav} ii(a) and  Theorem~\ref{thm: difference_equilibrium_behav_non_behav} i(c)). Thus, substituting in \eqref{eq: Security Under Anarchy} also yields that $PoBW = 1$.\footnote{SS: Why do we need all these special case analyses?  Aren't they covered by your analysis below?  In particular, what do you mean by the case for $A \rightarrow \infty$?  I would just remove these unless the following analysis does not capture them for some reason.  You don't have to do a special case for $A = 1$, since you are just providing a general bound.}  
%\footnote{SS: don't you also have this if $A = 1$?  Check carefully. Mus: If A = 1, \hat{r} = r^* for any possible case, I added it above and also add in Theorem 1 part i(c).}
Substituting from \eqref{eq: Non_Behavioral_defender_expected_loss} into \eqref{eq: Security Under Anarchy} yields 
\begin{equation*}
PoBW = \frac{\text{max} \left\{p_{1}(\hat{r}), A p_{2}(R - \hat{r})\right\}}{\text{max} \left\{p_{1}(r^*), A p_{2}(R - r^*)\right\}}.
\end{equation*}
We consider the following four possible sub-cases. To get the upper bound of PoBW, we will leverage the fact that $e^{-R} \leq p_1(r) \leq 1$ and $e^{-R} \leq p_2(r) \leq 1$ (from the proposition statement) as follows.

i) If $p_1(\hat{r}) > A p_2(R-\hat{r})$ and $p_1(r^*) > A p_2(R-r^*)$, then we have  
\begin{align*}
PoBW &{=} \frac{p_1(\hat{r})}{p_1(r^*)} \stackrel{(a)}{=} \frac{\exp(-\hat{r})}{\exp(-r^*)} 
\stackrel{(b)}{\leq} \exp(R).
\end{align*}
Note that (a) holds from the proposition statement and (b) holds since the numerator is upper bounded by $1$  and the denominator is lower bounded by $e^{-R}$.

ii) If $p_1(\hat{r}) \leq A p_2(R-\hat{r})$ and $p_1(r^*) \leq A p_2(R-r^*)$, then we have  
\begin{align*}
PoBW &{=} \frac{Ap_2(R - \hat{r})}{Ap_2(R - r^*)} = \frac{A\exp(-R + \hat{r})}{A\exp(-R + r^*)} %\stackrel{(d)}
{\leq} \exp(R).
\end{align*}

iii) If $p_1(\hat{r}) > A p_2(R-\hat{r})$ and $p_1(r^*) \leq A p_2(R-r^*)$, then we have  
\begin{align*}
PoBW &{=} \frac{p_1(\hat{r})}{Ap_2(R - r^*)} = \frac{\exp(-\hat{r})}{A\exp(-R + r^*)} \stackrel{(c)}{\leq} \frac{\exp(R)}{A}.
\end{align*}
Note that (c) holds since the numerator is upper bounded by $1$  and the denominator is lower bounded by $A e^{-R}$.
%\footnote{SS: why is this only lower bounded with $A <1$?  Why isn't it lower bounded by $Ae^{-R}$ regardless of $A$? Mus: Removed it. Sorry for this misconception.}

iv) If $p_1(\hat{r}) \leq A p_2(R-\hat{r})$ and $p_1(r^*) > A p_2(R-r^*)$, then we have  
\begin{align*}
PoBW &{=} \frac{Ap_2(R - \hat{r})}{p_1(r^*)} = \frac{A\exp(-R + \hat{r})}{\exp(-r^*)} \stackrel{(d)}{\leq} A\exp(R).
\end{align*}
Similarly, (d) holds since the numerator is upper bounded by $A$ %(when $A > 1$)\footnote{SS: why do you have to put this restriction on A?}  
and the denominator is lower bounded by $e^{-R}$.
% \footnote{SS: Just include $\leq$ in the above cases, not just $<$.  You don't need the rest of this discussion below.  Your above four cases, once you include $\leq$ will cover all possibilities.  In particular, you can get rid of this $\beta$ here and earlier.  Let me know if I am missing something.
% Mus: Done. That is correct, now there are 9 possibilities covered. Can you double check this!!
% }

\iffalse
Now, we study the remaining cases in which $\hat{r}(v)$ uniquely satisfies $w(p_1(\hat{r}(v),v)) = A w(p_2(R-\hat{r}(v)))$ and $r^*(v)$ uniquely satisfies $p_1(r^*(v),v) = A p_2(R-r^*(v))$. We start with studying the case at $A=1$, from Theorem~\ref{thm: difference_equilibrium_behav_non_behav}, $\hat{r}(v) = r^*(v)$. Substituting in \eqref{eq: Security Under Anarchy} yields that $PoBW = 1$. %Thus, PoBW is lower bounded by $1$. 

Finally, consider the cases of $A \neq 1$. Then, we have
\begin{align*}
PoBW &\stackrel{(e)}{=} \frac{\text{max} \left\{p_{1}(\hat{r}(v), v), A p_{2}(R - \hat{r}(v))\right\}}{\beta p_{1}(r^*(v), v) + (1 - \beta) A p_{2}(R - r^*(v))} \\ 
& \stackrel{(f)}{\leq} \frac{A}{A p_{2}(R - r^*(v))} 
\stackrel{(g)}{\leq} \exp(R).
\end{align*}
Note that (e) holds since $p_1(r^*(v),v) = A p_2(R-r^*(v))$ (i.e., both sites 1 and 2 would return same payoff to the attacker) and thus the  attacker strikes site 1 with any probability $\beta \in [0,1]$. Also, (f) holds since both $p_{1}(\hat{r}(v), v)$ and $p_{2}(R - \hat{r}(v))$ are upper bounded by $1$ and $A p_2(R- r^*(v)) = p_1(r^*(v),v)$ (from Assumption~\ref{ass: equalizing_rational}). Moreover, (g) holds since $p_2(R-r^*(v))$ is lower bounded by $\exp(-R)$.
\fi
%Note that (a) holds since the attacker is indifferent from Theorem~\ref{thm: difference_equilibrium_behav_non_behav}, we have $\hat{r}(v) > r^*(v)$ and thus from Proposition~\ref{prop: rational_attacker_decisions}, we have $A p_2(R- \hat{r}(v)) > p_1(\hat{r}(v),v)$ and (b) holds since $A p_2(R- r^*(v)) = p_1(r^*(v),v)$. Moreover, (c) holds from the statement of the proposition. Finally, we have $\hat{r}(v) > r^*(v)$ when $A < 1$ (from Theorem~\ref{thm: difference_equilibrium_behav_non_behav}). Then, The numerator is upper bounded by $1$. On the other hand, the denominator is lower bounded by $\exp(-R)$. Substituting these bounds into \eqref{eq: Security Under Anarchy}, we obtain (d) where $PoBW \le \exp(R)$.
 
\iffalse
Now, consider the case of $A > 1$ and $p_1(r^*(v),v) < \frac{1}{e}$. We have  
\begin{align*}
PoBW &= \frac{p_1(\hat{r}(v),v)}{\beta p_{1}(r^*(v), v) + (1 - \beta) A p_{2}(R - r^*(v))}\\
&= \frac{p_1(\hat{r}(v),v)}{p_1(r^*(v),v)} = \frac{\exp(r^*(v))}{\exp(\hat{r}(v))} \leq \exp(R).
\end{align*}
With a similar argument (and noting the fact that $\hat{r}(v) < r^*(v)$ when $A > 1$ (from Theorem~\ref{thm: difference_equilibrium_behav_non_behav})), we obtain $PoBW \le \exp(R)$. 
\fi
In all of the possible scenarios (as shown above), $PoBW \leq \max\{A, \frac{1}{A}\} \exp(R)$, which concludes the proof.
% \footnote{SS: this is vague.  The reader has no idea what $k$ is.  Your bounds are all in terms of $A$.  Just give an explicit characterization of the constant in terms of $A$.  Isn't it just something like $\max\{A, \frac{1}{A}\}$?} that concludes the proof.
% Mus: Changed it to $\max\{A, \frac{1}{A}\}$.
\end{proof}


Now, we illustrate our above characterizations of the impacts of behavioral decision-making via numerical simulations. 



==> Properties_Behavioral_Sequential_Game.tex <==
\section{Properties of the Behavioral Defender-Attacker Sequential Game}
\begin{comment}
\subsection{Convexity of the Objectives}
Here, we prove the convexity of the defender's cost function in the behavioral signaling games defined in Section \ref{sec:behavioralclasses}. Then, we study 

\begin{assumption} \label{ass: prob_attack}
The probability function $p_{1}(r,v)$ has the following properties.
\begin{itemize}
\item $p_{1}(r,v)$ is twice differentiable 
\item $p_{1}(r,v)$ is decreasing and log-convex\footnote{This is a common assumption in the literature. In particular, \cite{baryshnikov2012security} shows that log-convexity of the attack probability functions is a necessary and sufficient condition for the optimal security investment result of the seminal paper \cite{gordon2002economics} to
hold.} in $r$.
%\item p(x,y) is increasing and concave in $y$.
\end{itemize}
\end{assumption}
In other words, $p_{1}(r,v)$ is log-convex and decreasing with respect to defensive investment $r$ on site 1.

\begin{proposition}
Under Assumption 1, the behavioral defender's expected (perceived) loss $L_{w}(r,v)$ is convex in investments $r$.
\end{proposition}

\begin{proof}
\textcolor{red}{
Beginning with the perceived expected loss $L_{w}(r,\alpha)$ defined in \eqref{eq: Behavioral_defender_expected_loss}
\begin{equation*}
L_{w}(r, \beta) = \beta w(p_{1}(r, v)) + (1 - \beta)w(p_{2}(R - r)),
\end{equation*}
now, calculating the second derivative with respect to $r$ yields
\begin{equation*}
\begin{aligned}
\pdv[2]{L_{w}}{r} &=  \beta w''(p_{1}(r,v)) (\frac{\partial p_{1}}{\partial r})^{2} + \beta w'(p_{1}(r,v)) \pdv[2]{p_{1}}{r}  \\
&+ (1-\beta) w''(p_{2}(R-r)) (p'_{2})^{2}\\ 
&+(1-\beta) w'(p_{2}(R-r)) p''_{2}.
\end{aligned}
\end{equation*}
Since $w(\cdot)$ is increasing function, $p_{1}$ and $p_{2}$ are convex in $r$, it is clear that the second and fourth term are positive. Moreover, since $w''(\cdot)$ is positive (under Assumption 1), the first and third term are also positive. Therefore, $\pdv[2]{L_{w}}{r}$ is always positive.} 
\end{proof}
The above result shows that the non-linear perception of probability of attack does not affect the convexity of the resource allocation problem defined in the last section. 
\end{comment}


\subsection{Uniqueness of defender's (perceived) optimal investment strategy}
First, we prove that the behavioral defender's allocation that minimizes her perceived loss (as captured by \eqref{eq: Behavioral_defender_expected_loss}) is unique. We later use this to understand how behavioral probability weighting affects the investments of the defender.
%\footnote{SS: I don't know if SPNE is the right concept to study for this game.  The defender has a clear optimization objective, given by minimizing $L_w(r,v)$.  The attacker only has two options.  I would drop the SPNE stuff and just show that the defender's optimization problem (minimizing the objective in \eqref{eq: Behavioral_defender_expected_loss}) has a unique solution.  I have rephrased Prop 1.

% Mus: I agree with this. I also removed SPNE from the introduction as well. 
%}  

\begin{proposition}\label{prop: equilibria_behavioral_complete_info}
%Subgame perfect equilibria of the Behavioral Defender-Attacker Sequential Game exist, and the defender's allocation is the same in all of them. This allocation, $\hat{r}(v)$,
%minmaxes the attacker;\footnote{SS: I don't know if we should say that this minimaxes the attacker, since the defender does not know the attacker's actual utility function.  The defender is just trying to minimize it's own loss function. Mus: Removed it.}
%is the unique solution to $\displaystyle \min_{r\in [0,R]} \max\{w(p_{1}(r, v)), A w(p_{2}(R - r))\}$.
For any 
%fixed $v \in \mathbb{R}_{> 0}$ and
$\alpha \in (0,1]$, the defender's optimal allocation to site $1$ in order to minimize $L_w(r)$ in \eqref{eq: Behavioral_defender_expected_loss} is unique, and denoted by $\hat{r}$.
\end{proposition}

\begin{proof}
First, note that since $w(p)$ is strictly increasing in $p$, and by our assumption that $p_1(r)$ is strictly decreasing in $r$, we have that $w(p_1(r))$ is strictly decreasing in $r$.  Similarly, by our assumption that $p_2(x)$ is strictly decreasing in its argument, the function $p_2(R-r)$ is strictly increasing in $r$.  Thus, $Aw(p_2(R-r))$ is strictly increasing in $r$.
%\footnote{SS: you don't need all of the derivatives.  Just use the fact that $w$ is increasing in its argument.  I have rewritten this part.
% Mus: I see. Thanks.
%}

\iffalse
We first show that $w(p_1(r,v))$ is decreasing in $r$ and $A w(p_2(R-r))$ is increasing in $r$ as follows.
\begin{equation*}
\frac{\partial w(p_1(r,v))}{\partial r}  = \frac{\alpha w(p_1(r,v))}{p_1(r,v)} \left[ -\log(p_1(r,v)) \right]^{\alpha - 1} \frac{\partial p_1(r,v)}{\partial r}.
\end{equation*}
In the derivative $\frac{\partial w(p_1(r,v))}{\partial r}$, we have $0 \leq p_1(r,v) \leq 1$, thus we have $-\log(p_1(r,v)) \in R_{\geq 0}$. Moreover, both $\alpha$ and $w(\cdot)$ are non-negative. On the other hand, we have $\frac{\partial p_1(r,v)}{\partial r} < 0$, thus we have $\frac{\partial w(p_1(r,v))}{\partial r} < 0$. Similarly, it is easy to show that $\frac{dw(p_2(R-r))}{dr} > 0$.
\fi

% s in which $w(p_{1}(\hat{r}(v), v)) \neq A w(p_{2}(R - \hat{r}(v)))$. 

First, consider the case where
%where $A$ is very large such that
$w(p_{1}(r)) < A w(p_{2}(R-r)) \forall r \in [0,R]$. Then, $\hat{r} = 0$ is the unique solution that minimizes the defender's perceived expected loss (since if the defender deviates to any investment $r > 0$, the defender's perceived expected loss $A w(p_{2}(R - r))$ would be larger as $Aw(p_2(R-r))$ is increasing in $r$). %$\frac{dw(p_2(R-r))}{dr} > 0$). 

Second, consider the case in which  $w(p_{1}(r)) > A w(p_{2}(R-r)) \forall r \in [0,R]$. Then, $\hat{r} = R$ is the unique solution that minimizes the defender's perceived expected loss (since if the defender deviates to any investment $r < R$, the defender's perceived expected loss $w(p_{1}(r))$ would increase as $w(p_1(r))$ is decreasing in $r$ as shown earlier). 

Now, consider the cases that are not considered by the above two (corner) cases. Note that since $w(p_1(r))$ is strictly decreasing in $r$, and since $Aw(p_2(R-r))$ is strictly increasing in $r$, and since neither function is always larger than the other (which was captured by the previous two cases), there must be a unique value of $r$ at which $w(p_{1}(r)) = A w(p_{2}(R - r))$.  This will be the unique solution to the problem of minimizing \eqref{eq: Behavioral_defender_expected_loss}, which we denote by $\hat{r}$.
%\footnote{SS: your previous argument  was incomplete.  How do you know that there is a single value of $r$ that equalizes the two functions?  What happens if there are multiple crossings?   You have to argue that the first function is strictly decreasing and the second function is strictly increasing.  I have now fixed this everywhere.  I also removed the rest of the proof, as it was trivial.
% Mus: I see. Thanks for the fix.%}
%To establish that the only equilibrium allocation is $\hat{r}(v)$, following the argument of \cite{powell2007allocating}, suppose by contradiction that the defender can profitably deviate from any $r' \neq \hat{r}(v)$. Assume, first, that $r < \hat{r}(v)$. Then the defender is spending too little on site 1 such that: $w(p_{1}(r, v)) > A w(p_{2}(R - r))$. The defender perceives that the attacker therefore would hit site 1, which leaves the defender with an expected loss of $w(p_{1}(r, v))$ whenever $r < \hat{r}(v)$. Hence, the defender can profitably deviate to any $r'$ between $r$ and $\hat{r}(v)$ because $w(p_{1}(r, v)) > w(p_{1}(r', v))$ for all $r' \in (r,\hat{r}(v))$ as $w(p_{1}(r, v))$ is decreasing in r (as shown in the beginning of the proof).
%Conversely, if the defender is spending too much on site 1 when $r > \hat{r}(v)$ and, as a result, we have $A w(p_{2}(R - r)) > w(p_{1}(r, v))$ when $r > \hat{r}(v)$. Then, if the attacker consequently strikes site 2 whenever $r > \hat{r}(v)$, the defender's perceived expected loss would be $A w(p_{2}(R - r))$. Now the defender can profitably deviate from $r$ to any $r'$ between $\hat{r}(v)$ and $r$. From the above scenarios, the only possible equilibrium allocation is $\hat{r}(v)$.
\end{proof}


\begin{figure}%[b]
\begin{center}
  \includegraphics[width=0.75\linewidth]{Figures/Complete_info_resource_payoff.eps}
  \caption{An illustration of the defender's minmax problem under misperception of the probabilities of successful attack on each site.}
  \label{fig:Payoff vs resources on site 1}
\end{center}
\end{figure}

Fig. \ref{fig:Payoff vs resources on site 1} illustrates $\hat{r}$, i.e., the allocation that minimizes the maximum perceived expected loss for the defender.
%\footnote{SS: The figure does not show $\hat{r}(v)$.  Mark it on the figure.  Also, the y axis of the figure says expected payoff for the attacker.  Isn't this the expected perceived loss of the defender for each site?
% Mus: Thanks for the comment. I modified the figure.
%}

%Formally, $\hat{r}(v)$ solves $\min_{r\in [0,R]} \max\{w(p_{1}(r, v)), A w(p_{2}(R - r))\}$, and is what the behavioral defender does in any sub game perfect equilibrium. 

\subsection{Effect of probability weighting on the defender's investment strategy}
We now characterize the impact of probability weighting  on  the defender's investments in each of the two sites.  To aid in our analysis, let us define the difference function between the defender's losses in the two sites as $ D(r) = w(p_{1}(r)) - A w(p_{2}(R - r))$.  As argued earlier, since the first term is strictly decreasing in $r$ and the second term $(Aw(p_2(R-r)))$ is strictly increasing in $r$, we see that $D(r)$ is strictly decreasing in $r$. In particular, $D(r)$ is positive if $w(p_{1}(r)) >  A w(p_{2}(R - r))$, negative  if $w(p_{1}(r)) <  A w(p_{2}(R - r))$, and zero if $w(p_{1}(r)) =  A w(p_{2}(R - r))$. 


\iffalse
\begin{corollary}\label{cor: difference_decreasing}
Let $ D(r) = w(p_{1}(r, v)) - A w(p_{2}(R - r))$, then $D(r)$ is decreasing in $r$.
\end{corollary}
\begin{proof}
The proof follows by differentiating $D(r)$ w.r.t. $r$ as follows:
\begin{equation*}
    D'(r) = w'(p_{1}(r, v)) \frac{\partial{p_1(r,v)}}{\partial {r}}\ + A w'(p_{2}(R - r)) p'_{2}(R - r).
\end{equation*}
Since $w(\cdot)$ is increasing, $w'(\cdot)$ is positive. Moreover, we have $\frac{\partial{p_1(r,v)}}{\partial {r}} < 0$ and $p'_{2}(R - r) < 0$. Therefore, $D'(r)$ is negative and thus $D(r)$ is decreasing in $r$.  
\end{proof}
\fi


Now, we show how the investment by the defender in site $1$ changes under behavioral probability weighting.  In order to keep the exposition clear, we will make the following assumption on the probabilities and site values for the case where there is no probability weighting (this assumption rules out the two corner cases where a non-behavioral defender invests entirely in only one of the two sites).  This assumption was also made in \cite{powell2007allocating}.

\begin{assumption}\label{ass: equalizing_rational}
The quantities $p_1(r)$ and $Ap_2(R-r)$ are such that $p_1(0) > Ap_2(R)$ and $p_1(R) < Ap_2(0)$, i.e., there is a unique quantity $r^*$ such that $p_{1}(r^*) = A p_{2}(R - r^*)$.
\end{assumption}


\begin{theorem}\label{thm: difference_equilibrium_behav_non_behav}
Consider a behavioral defender (with $\alpha \in (0,1)$) that faces losses of $1$ and $A$ if the sites 1 and 2  are successfully compromised, respectively. Let $\hat{r}$ be the defender's allocation that minimizes its loss \eqref{eq: Behavioral_defender_expected_loss}, where $\hat{r}$ is defined in Proposition~\ref{prop: equilibria_behavioral_complete_info}. Moreover, let $r^*$
be the non-behavioral (with $\alpha = 1$) defender's optimal allocation that satisfies Assumption~\ref{ass: equalizing_rational}. %given by the unique solution to $\displaystyle r^*(v) = \arg \min_{r\in [0,R]} \max\{p_{1}(r, v), A p_{2}(R - r)\}$. 
We have the following cases.
\begin{enumerate}
    \item If $\hat{r}$ does not satisfy $w(p_1(\hat{r})) = A w(p_2(R-\hat{r}))$, and
        \begin{enumerate}
        \item If $w(p_1(r)) < A w(p_2(R-r)) \forall r\in [0,R]$, then $\hat{r} \leq r^*$.
        \item If $w(p_1(r)) > A w(p_2(R-r)) \forall r\in [0,R]$, then $\hat{r} \geq r^*$.
        %\item In both of the cases i(a) and i(b), if $A = 1$, then $\hat{r} = r^*$.
        \end{enumerate}

    \item If $\hat{r}$ satisfies $w(p_1(\hat{r})) = A w(p_2(R-\hat{r}))$, and
        \begin{enumerate}
        \item If $A = 1$, then $\hat{r} = r^*$,
        \item If $p_{1}(r^*) < \frac{1}{e}$ and $A < 1$, then  $\hat{r} > r^*$,
        \item If $p_{1}(r^*) < \frac{1}{e}$ and $A > 1$, then $\hat{r} < r^*$.
    \end{enumerate}
\end{enumerate}
\end{theorem}

\begin{proof}
We begin with the cases in which the behavioral defender cannot equalize the perceived losses.  In the case i(a) where $w(p_{1}(r)) < A w(p_{2}(R-r)) \forall r \in [0,R]$, we have $\hat{r} = 0$ from  Proposition~\ref{prop: equilibria_behavioral_complete_info}. Thus, we have $r^* \geq \hat{r}$.
In the case i(b) in which $w(p_{1}(r)) > A w(p_{2}(R-r)) \forall r \in [0,R]$, we have $\hat{r} = R$ from Proposition~\ref{prop: equilibria_behavioral_complete_info}.  Thus, we have $r^* \leq \hat{r}$. %Then, the case i(c) follows when $A = 1$ from the fact that $w(p)$ is a strictly increasing function of $p$ as mentioned earlier in Section~\ref{sec:behavioraprelec}.


Now, consider the remaining cases, that are not considered by the above (corner) cases, where
$\hat{r}$ uniquely satisfies $w(p_{1}(\hat{r})) = A w(p_{2}(R - \hat{r}))$. %\footnote{SS: What if you cannot equalize?  Again, please make sure that you go through the whole paper carefully.} 
%From \cite{powell2007allocating}, $r^*(v)$ satisfies $p_{1}(r^*(v), v) = A p_{2}(R - r^*(v))$. 

Recall that $D(r) = w(p_{1}(r)) - Aw(p_{2}(R - r)) $ and thus we have $D(\hat{r}) = 0$. Also, from Assumption~\ref{ass: equalizing_rational}, $r^*$ satisfies the relation
$p_{1}(r^*) = A p_{2}(R - r^*)$.   
Thus, 
\begin{align}
D(r^*) &= w(p_{1}(r^*)) - Aw(p_{2}(R - r^*)) \nonumber\\
&= w(p_{1}(r^*)) - A w\left(\frac{p_{1}(r^*)}{A}\right). \label{eq:Drstar}
\end{align}
Now, we prove the following three cases:


Case ii(a): If $A = 1$, 
 we have $D(r^*) = 0$. 
 However, from Proposition~\ref{prop: equilibria_behavioral_complete_info},  $\hat{r}$ is the  defender's unique investment strategy that satisfies $w(p_1(r)) = A w(p_2(R - r))$ (i.e., $\hat{r}$ is the only investment that satisfies $D(\hat{r}) = 0$). Therefore, $\hat{r} = r^*$. In other words, the defense allocations of behavioral and non-behavioral defenders are identical if $A = 1$. 
 %Second, if $r < \hat{r}(v)$, $w(p_{1}(r, v)) >  w(p_{2}(R - r))$ and w(.) is an increasing function so $p_{1}(r, v) > p_{2}(R - r)$. Finally, with similar argument, if $r > \hat{r}(v)$, $w(p_{2}(R-r)) >  w(p_{1}(r,v))$ and therefore $p_{2}(R - r) > p_{1}(r,v)$. 
 
 Now, for the other cases in ii(b) and ii(c), we show that $\hat{r} \neq r^*$ (i.e., the optimal defense allocations are different for behavioral and non-behavioral defenders). %Suppose by contradiction that $\hat{r}(v) = r^*(v)$ (i.e., the optimal defense allocation is equivalent for both behavioral and non-behavioral defenders). However,
%From Proposition \ref{prop: equilibria_behavioral_complete_info}, $\hat{r}(v)$ satisfies the following relation
Recall that since $w(p_{1}(\hat{r})) = A w(p_{2}(R - \hat{r}))$, 
% \begin{equation}\label{eq: payoffs_equality_differentlosses}
% w(p_{1}(\hat{r}(v), v)) = A w(p_{2}(R - \hat{r}(v))).
% \end{equation}
we have $D(\hat{r}) = 0$. 
% \begin{equation}\label{eq: rational_payoffs_equality_differentlosses}
%  p_{1}(r^*(v), v) = A p_{2}(R - r^*(v)).
% \end{equation} 
%Now, applying $w^{-1}(\cdot)$ for both sides in Equation~\eqref{eq: payoffs_equality_differentlosses}, we have $p_{1}(\hat{r}(v), v) = w^{-1}(A w(p_{2}(R - \hat{r}(v)))) \neq A p_{2}(R - \hat{r}(v))$ which yields a contradiction and shows that $\hat{r}(v) \neq r^*(v)$. 
%From ~\eqref{eq: rational_payoffs_equality_differentlosses}, we have, $w(p_{1}(r^*(v), v)) = w(A p_{2}(R - r^*(v)))$. 
To show that $\hat{r} > r^*$, it is sufficient to show that $D(r^*) > 0$ (since $D(r)$ is strictly decreasing in $r$). Similarly, to show that $\hat{r} < r^*$, it is sufficient to show that $D(r^*) < 0$.

For ease of notation, we will drop the argument $r^*$ of $p_1$ in the following steps of the proof.  We first substitute the form of the Prelec function from \eqref{eq:prelec} into \eqref{eq:Drstar} to obtain
\begin{align*}
D(r^*) &= e^{-(-\log(p_1))^{\alpha}} -A e^{-(\log(A)-\log(p_{1}))^{\alpha}}. \\ 
&= e^{-(-\log(p_1))^{\alpha}}  \left[ 1 - A y(\alpha)\right],
\end{align*}
\begin{comment}
ii) If $A < 1$, we have
\begin{align*}
 A < 1 \iff & -\log(p_1)+\log(A) < -\log(p_1)\\ 
% \iff & (-\log(p_1)+\log(A))^{\alpha} < (-\log(p_1))^{\alpha}\\
% \iff & -(-\log(p_1)+\log(A))^{\alpha} > -(-\log(p_1))^{\alpha}\\
% \iff & e^{-(-\log(p_1)+\log(A))^{\alpha}} > e^{-(-\log(p_1))^{\alpha}}\\
 \iff & (-\log(p_1)+\log(A))^{\alpha-1} > (-\log(p_1))^{\alpha - 1}
\end{align*}
\end{comment}
where $y(\alpha) = e^{-(\log(A)-\log(p_{1}))^{\alpha} + (-\log(p_{1}))^{\alpha}}$. %ii) If $A < 1$, we have

Case ii(b): We prove this case by dividing it into two sub-cases as follows. First, we consider the sub-case where $p_1 < \frac{1}{e}$ and $A \in (e p_1 , 1)$. We first differentiate $y(\alpha)$ w.r.t. $\alpha$ to get 
% \footnote{SS: i haven't checked this derivation.  Please make sure it is correct.  Also, one thing that is unclear: the derivative does not care about your conditions on $A$ and $p_1$ that you placed in the theorem.  But if $\frac{A}{p_1}$ is less than $e$, then $\log \log \frac{A}{p_1}$ does not exist.  So what happens to the derivative in those situations? Mus: added below after our discussion via email that " Note that $\frac{dy(\alpha)}{d\alpha}$ exists (since from \eqref{eq:Drstar} $p_1(r^*) \leq A$ and thus all the $\log$ terms exists)".}
\begin{align*}
    \frac{dy(\alpha)}{d\alpha} &= y(\alpha) \big[-\left(\log(\frac{A}{p_1})\right)^{\alpha} \log(\log(\frac{A}{p_1}))  \\  
    &+ \left(\log(\frac{1}{p_1})\right)^{\alpha} \log(\log(\frac{1}{p_1}))\big].
\end{align*}
Note since $p_1 < \frac{1}{e}$, we have $\log(\frac{1}{p_1}) > 1$
%\footnote{SS: should this be bigger than 1?} % Mus: Correct, I modified it in several places here, but the earlier was sufficient for the sign of the derivative to be positive.
and $\log(\log(\frac{1}{p_1})) > 0$. Moreover, since $A \in (e p_1, 1 )$, we have $\log(\frac{A}{p_1}) > 1$ and $\log(\log(\frac{A}{p_1})) > 0$. Furthermore, 
\begin{align*}
 A \in (e p_1, 1) \iff & \log(\frac{A}{p_1}) < \log(\frac{1}{p_1})\\ 
\iff & \left(\log(\frac{A}{p_1})\right)^{\alpha} < \left(\log(\frac{1}{p_1})\right)^{\alpha}\\
\iff & \log(\log(\frac{A}{p_1})) < \log(\log(\frac{1}{p_1})).
\end{align*}
From the above inequalities and the fact that $y(\alpha) > 0$, we see that $\frac{dy(\alpha)}{d\alpha}$ is positive. In other words, $y(\alpha)$ is increasing in $\alpha$ and upper bounded at $\alpha = 1$ and therefore $y(\alpha) < y(1) = \frac{1}{A}$ for any $\alpha \in (0,1)$.  
Therefore, $D(r^*) > 0$. Finally, since $D(r)$ is strictly decreasing in $r$ and we have $D(\hat{r}) = 0$, we have $\hat{r} > r^*$.  

Now, we consider the second sub-case where $p_1 < \frac{1}{e}$ and $A \in (0, e p_1]$. In this sub-case, we use \eqref{eq:Drstar} to prove that $D(r^*) > 0$ as follows:
\begin{align*}
 D(r^*)  &= w(p_1) - A w\left(\frac{p_1}{A}\right)\\ 
 & \stackrel{(a)}{>} p_1 - A w\left(\frac{p_1}{A}\right) \\
 & \stackrel{(b)}{\geq} p_1 - A \frac{p_1}{A} = 0.
\end{align*}
Note that (a) holds since $p_1 < \frac{1}{e}$ and thus $w(p_1) > p_1$. Also, (b) holds since $A \in (0, e p_1]$, we have $\frac{p_1}{A} \geq \frac{1}{e}$ and thus we have $w\left(\frac{p_1}{A}\right) \leq \frac{p_1}{A}$.
Therefore, $D(r^*) > 0$, and thus we have $\hat{r} > r^*$.  

Case ii(c): We now prove the case when $A > 1$ as follows. In the derivative $\frac{dy(\alpha)}{d \alpha}$ (which always exists here since $A > 1$ and $p_1 < \frac{1}{e}$), since $p_1 < \frac{1}{e}$, we have $\log(\frac{1}{p_1}) > 1$ and $\log(\log(\frac{1}{p_1})) > 0$. Moreover, since $A > 1$ and $p_1 < \frac{1}{e}$, we have $\log(\frac{A}{p_1}) > 1$ and $\log(\log(\frac{A}{p_1})) > 0$. Moreover, 
\begin{align*}
 A > 1 \iff & \log(\frac{A}{p_1}) > \log(\frac{1}{p_1})\\ 
\iff & \left(\log(\frac{A}{p_1})\right)^{\alpha} > \left(\log(\frac{1}{p_1})\right)^{\alpha}\\
\iff & \log(\log(\frac{A}{p_1})) > \log(\log(\frac{1}{p_1})).
\end{align*}
From the above inequalities and the fact that $y(\alpha) > 0$, we have $\frac{d y(\alpha)}{d\alpha}$ is negative. In other words, $y(\alpha)$ is decreasing in $\alpha$ and lower bounded at $\alpha = 1$ and therefore $y(\alpha) > y(1) = \frac{1}{A}$ for any $\alpha \in (0,1)$.  

\iffalse
Now, we differentiate $y(\alpha)$ w.r.t. $p_1$ as follows. %and w.r.t $\alpha$ as follows
\begin{equation*}
    \frac{\partial y(\alpha)}{\partial p_1} = \frac{\alpha y(p_1)}{p_1}\left[ (\log(A)-\log(p_{1}))^{\alpha-1} - (-\log(p_{1}))^{\alpha-1}\right].
\end{equation*}
\begin{align*}
 A > e \iff & -\log(p_1)+\log(A) > -\log(p_1)\\ 
 \iff & (-\log(p_1)+\log(A))^{\alpha-1} < (-\log(p_1))^{\alpha - 1}.
\end{align*}
Thus, $y'(p_1)$ is negative and $y(p_1)$ is decreasing in $p_1$ and since $0 < p_1 \leq 1$, $y(p_1) \geq y(1) = e^{-(\log(A))^{\alpha}} \stackrel{(b)}{>} \frac{1}{A}$. Note that (b) holds since 
\begin{align*}
 A > e \iff & [\log(A)]^{\alpha} < \log(A) \\ 
 \iff & -[\log(A)]^{\alpha} > -\log(A) \\
 \iff & e^{-(\log(A))^{\alpha}} > e^{-(\log(A))} = \frac{1}{A}.
\end{align*}
%at $A > e$, $e^{-(\log(A))^{\alpha}}$ is a decreasing function in $\alpha$ (i.e.,  $\displaystyle \frac{d}{d\alpha} (e^{-(\log(A))^{\alpha}}) = - (\log(A))^{\alpha} \log(\log(A))  e^{-(\log(A))^{\alpha}}$ is negative) and thus $e^{-(\log(A))^{\alpha}}$ is lower bounded at $\alpha = 1$. 
\fi
Therefore, $D(r^*) < 0$. Again, since $D(r)$ is strictly decreasing in $r$, and we know that $D(\hat{r}) = 0$, we have $\hat{r} < r^*$. That concludes the proof.  
\iffalse
We have $\alpha > 0$, $p_1 > 0$, and $y(p_1) > 0$. Moreover, we have:
\begin{align*}
ii) A < 1 \iff & -\log(p_1)+\log(A) < -\log(p_1)\\ 
 \iff & (-\log(p_1)+\log(A))^{\alpha-1} > (-\log(p_1))^{\alpha - 1}
\end{align*}

Note that the last inequality holds since $0 < \alpha < 1$. Thus, $y'(p_1)$ is positive and $y(p_1)$ is increasing in $p_1$ and since $0 < p_1 \leq 1$, $y(p_1) < y(1) = e^{-(\log(A))^{\alpha}} \stackrel{(a)}{<} \frac{1}{A}$. 
\fi
%Note that (a) holds since at $A < 1$, $e^{-(\log(A))^{\alpha}}$ is an increasing function
%\footnote{Let $z(\alpha) = e^{-(\log(A))^{\alpha}}$, then we have $\displaystyle z'(\alpha) = - (\log(A))^{\alpha} \log(\log(A))  e^{-(\log(A))^{\alpha}}$.}
%in $\alpha$ and upper bounded at $\alpha = 1$. Therefore, $D(r^*(v)) > 0$. Finally, since $D(r)$ is decreasing in $r$, 
%(from Corollary~\ref{cor: difference_decreasing}), 
% and we have $D(\hat{r}(v)) = 0$, thus we have $\hat{r}(v) > r^*(v)$.
\end{proof}

\begin{figure*}[hbt!]%[t]
\centering
\begin{minipage}[t]{1.0\textwidth}
\begin{minipage}[t]{.45\textwidth}
\centering
 \includegraphics[width=0.9\linewidth]{Figures/Shift_figure_A_less_than_one.eps}
  \caption{The effect of behavioral probability weighting on the defender's investments with $A < 1$.}
  \label{fig:investments_A_less_than_one}
\end{minipage}\hfill
\begin{minipage}[t]{.45\textwidth}
\centering
  \includegraphics[width=0.9\linewidth]{Figures/Shift_figure_A_greater_than_one.eps}
  \caption{The effect of behavioral probability weighting on the defender's investments with $A > 1$.}
  \label{fig:investments_A_greater_than_one}
\end{minipage}
\end{minipage}
\end{figure*}


The above result shows that the optimal defense allocations for both behavioral and non-behavioral defenders are different if $A \neq 1$ (i.e., the sites have different financial losses when compromised). In other words, the behavioral defender allocates more resources to the higher valued site compared to the non-behavioral defender (recall that $\hat{r}$ is the amount of defense resources allocated by the behavioral defender on site 1). This is illustrated in Fig.~\ref{fig:investments_A_less_than_one}, where the second site has a smaller value and therefore $\hat{r} > r^*$ (i.e., the behavioral defender allocates more resources on site 1).  On the other hand, if $A > 1$ (as shown in Fig.~\ref{fig:investments_A_greater_than_one}) the second site has a higher value and therefore $\hat{r} < r^*$. To generate those figures, we use $p_1(r) = \exp(0.5-r)$, $p_2(r) = \exp(-(R-r))$ and $R = 6$. 
%\footnote{SS: have you verified that the $A$ and $r^*$ in those figures satisfy the additional conditions that you imposed in the theorem? 
% Mus: Yes, here in Fig. 3, $A=0.5$ while $p_1(r^*) < 0.1$ and in Fig. 4 also $p_1(r^*) < \frac{1}{e}$. Also, assumption 1 is satisfied.  
%SS: Also, you should state what $p_1(r,v)$ and $p_2(R-r)$ you used for these figures.  Finally, use the word ``asset'' or ``site'' consistently.  The figure says asset, but we've been using site up to now.  Either one is fine.
% Mus: Added at the end of the paragraph.
%}
% \footnote{SS: You have not discussed what happens if the extra restrictions that you put on $A$ and $p_1(r^*)$ in the theorem do not hold.  You should put a discussion of that here.  In particular, intuitively it seems that in case ii(b), if $A$ is even smaller than the lower bound you put on it, the same result should hold.  Is there a different special case analysis you can do for this situation?  Otherwise, it seems somewhat arbitrary to put such a constraint on $A$.
% Mus: I'm updating Thm 1 and Prop 2 to be for any A < 1.
%}    

\iffalse
%% Commented for CDC Final Version
\subsection{Effect of defender's misperception on the attacker's choice}
The above result of Theorem~\ref{thm: difference_equilibrium_behav_non_behav} brings us to the following result, establishing the effect of the behavioral defender's investment on the attacker's choice of targets. In this context, we study that effect by considering the attacker's move in the sequential game. We will show that when facing a behavioral defender and under the scenarios (mentioned in Theorem~\ref{thm: difference_equilibrium_behav_non_behav}) where the two sites have different loss values to the defender, the attacker always has a strict preference on which site to strike (in contrast to the situation with a non-behavioral defender, where the defense investments make the attacker indifferent between the sites).
% \footnote{SS: what if $A = 1$? Mus: added "and under the scenarios (mentioned in Theorem~\ref{thm: difference_equilibrium_behav_non_behav}) where the two sites have different losses to the defender."} 
Correspondingly, we show that the behavioral defender's investment strategy shown in Theorem~\ref{thm: difference_equilibrium_behav_non_behav} yields an increase in her true expected loss (i.e., the attacker's payoff would be higher against a behavioral defender, when compared to a non-behavioral defender). 

Recall from the Behavioral Defender-Attacker Sequential Game  in Section~\ref{sec:behavioralclasses} that the attacker observes the defender's investment on site 1 and then chooses to hit the site that offers her a higher payoff. Let us define the function $E(r) = p_{1}(r) - A p_{2}(R - r)$. Note that 
if $E(r) > 0$, the non-behavioral attacker would hit site 1,  if $E(r) < 0$, the non-behavioral attacker would hit site 2, and if $E(r) = 0$, the non-behavioral attacker is indifferent between the sites. It is easy to see that $E(r)$ is strictly decreasing with $r$. 
%, and hits site 1 with some probability $\beta \in [0,1]$. 
\begin{proposition}\label{prop: rational_attacker_decisions}
Consider a behavioral defender (with $\alpha < 1$), and suppose the allocation $\hat{r}$ on site 1 is such that $w(p_{1}(\hat{r})) = A w(p_{2}(R - \hat{r}))$.
Let the losses on sites 1 and 2 (when compromised) be 1 and $A$, respectively. Moreover, let $r^*$ be the non-behavioral (with $\alpha = 1$) defender's optimal allocation that satisfies Assumption~\ref{ass: equalizing_rational}. Then,
%given by the unique solution that satisfy $p_{1}(r, v) = A p_{2}(R - r)$. Then,
\begin{enumerate}
\item If $p_{1}(r^*) < \frac{1}{e}$ and $A < 1$, the attacker would hit site 2.
\item If $p_1(r^*) < \frac{1}{e}$ and $A > 1$, the attacker would hit site 1.
\item In both of (i) and (ii), the attacker would have higher payoff compared to facing a non-behavioral defender (with $\alpha = 1$). Formally, $U(\hat{r}) > U(r^*)$.  
\end{enumerate}
\end{proposition}

\begin{proof}
(i) If $p_{1}(r^*) < \frac{1}{e}$ and $A < 1$, we have $\hat{r} > r^*$ (from Theorem~\ref{thm: difference_equilibrium_behav_non_behav}). By our assumptions that $p_1(r)$ is strictly decreasing in $r$ and $p_2(R-r)$ is strictly increasing in $r$, we have $p_1(\hat{r}) < p_1(r^*)$ and $A p_2(R- \hat{r}) > A p_2(R- r^*)$. Thus, we have $A p_2(R- \hat{r}) > p_1(\hat{r})$ (from the fact that $A p_2(R- r^*) = p_1(r^*)$). Therefore, $E(\hat{r}) < 0$ and the attacker would hit site 2. 

(ii) Second, if $p_1(r^*) < \frac{1}{e}$ and $A > 1$, we have $\hat{r} < r^*$ (from Theorem~\ref{thm: difference_equilibrium_behav_non_behav}). With a similar argument to (i), we have $A p_2(R- \hat{r}) < p_1(\hat{r})$. Thus, $E(\hat{r}) > 0$ and the attacker would hit site 1. 

(iii) Now, we compare the attacker's payoff under the defense investments $r^*$ and $\hat{r}$ by the non-behavioral and behavioral defender, respectively.

If $p_{1}(r^*) < \frac{1}{e}$ and $A < 1$, we have 
\begin{align*}
 \hat{r} > r^* \iff & A p_2(R- \hat{r}) > A p_2(R- r^*) \\  
 \iff & U(\hat{r}) \stackrel{(a)}{>} U(r^*).
\end{align*} 
Note that (a) holds since $A p_2(R- r^*) = p_1(r^*)$ (from Assumption~\ref{ass: equalizing_rational}) and $A p_2(R- \hat{r}) > p_1(\hat{r})$ (from (i)) and by substituting in \eqref{eq: Behavioral_attacker_utility}.

Second, if $p_{1}(r^*) < \frac{1}{e}$ and $A > 1$, we have 
\begin{align*}
 \hat{r} < r^* \iff & p_1(\hat{r}) > p_1(r^*) \\  
 \iff & U(\hat{r}) \stackrel{(b)}{>} U(r^*).
\end{align*}
Similarly, (b) holds since $A p_2(R- r^*) = p_1(r^*)$ and $A p_2(R- \hat{r}) < p_1(\hat{r})$ (from (ii)).
%Thus, in both of the possible cases of $A$, the non-behavioral attacker would have higher payoff when facing behavioral defender (with $\alpha_{\mathcal{D}} <1$).
\end{proof}

The above result shows that under loss asymmetry, the non-behavioral attacker benefits (i.e., has a higher payoff) from the behavioral defender's investment decisions. In the next section, we will seek to quantify this increase in the attacker's payoff (or equivalently, the increase in the defender's {\it true} expected loss).
\fi



\iffalse
\begin{remark}
Note that if defender is non-behavioral (with $\alpha = 1$). From \cite{powell2007allocating}, the non-behavioral defender allocates $r^*(v)$ to site 1 such that $A p_2(R- r^*(v)) = p_1(r^*(v),v)$. That makes the non-behavioral attacker indifferent between the two sites to maximize her expected returns (since both sites 1 and 2 would return same payoff to the attacker). Thus, the non-behavioral attacker strikes site 1 with any probability $\beta \in [0,1]$. We will use this fact later in our discussions.
\end{remark}
\fi

%the attacker hits site 1 if $r < \hat{r}(v)$; site 2 if $r > \hat{r}(v)$; and strikes site 1 with any probability $\beta \in [0,1]$ if $r = \hat{r}(v)$. 

%% Figures of Shift of optimal investments


\iffalse
\subsection{Dependence of allocation on vulnerability level}
Now, we study the effect of vulnerability level for the defender's optimal defense allocation. 
\begin{corollary}
The rate of change of defense allocation in site 1 with respect to vulnerability for  behavioral defender $\frac{d \hat{r}(v)}{dv}$ is different from the rate of change of defense allocation in site 1 with respect to vulnerability for  non-behavioral defender $\frac{d r^*(v)}{dv}$. Formally, $\frac{d \hat{r}(v)}{dv} \neq \frac{d r^*(v)}{dv}$.
%In both cases, the more vulnerable site I, the more the defender allocates to that site when there is complete information about vulnerability.
\end{corollary}

\begin{proof}
We would use implicit differentiation in both scenarios. First, in the case of non-behavioral defender (with $\alpha = 1$), using implicit differentiation of \eqref{eq:optimal_defense_allocation_powel_paper} the rate of change of defense allocation in site 1 with respect to vulnerability $\frac{d r^*(v)}{dv}$ is
\begin{equation}\label{eq:rate_change_rational}
\frac{d r^*(v)}{dv} = - \frac{\frac{\partial p_{1}}{\partial v}}{\frac{\partial p_{1}}{\partial r} + A p'_{2}}.
\end{equation}
Second, in the case of a behavioral defender (with $\alpha < 1$), using implicit differentiation of \eqref{eq: payoffs_equality_differentlosses} $\frac{d \hat{r}(v)}{dv}$ is given by
\begin{equation}\label{eq:rate_change_behavioral}
\frac{d \hat{r}(v)}{dv} = - \frac{\frac{\partial p_{1}}{\partial v}}{\frac{\partial p_{1}}{\partial r} + A p'_{2} \frac{w'(p_{2}(r))}{w'(p_{1}(r,v))}}.
\end{equation}
It is clear from \eqref{eq:rate_change_behavioral} that the rate of change of misperception of probability functions $p_{1}$ and $p_{2}$ affect the rate $\frac{d \hat{r}(v)}{dv}$. 
\end{proof}

Note that since $\frac{\partial p_{1}}{\partial v} > 0$, $\frac{\partial p_{1}}{\partial r} < 0$ and $p'_{2} < 0$. Thus, $\frac{d r^*(v)}{dv}$ in \eqref{eq:rate_change_rational} is positive. Also, both $w'(p_{2}(r))$ and $w'(p_{1}(r,v))$ have positive sign and thus \eqref{eq:rate_change_behavioral} is also positive. In other words, regardless the behavioral level of the defender, the more vulnerable site 1, the more the defender allocates to that site.
\fi

%This brings us to the following result, establishing the existence of a PNE in the Multi-Targets Behavioral Security Games. Recall that a set of security investments is said to be a PNE if no player can decrease her cost (or increase her utility) by unilaterally changing her investment.


